Evaluating Interactive Summarization: an Expansion-Based Framework

Allowing users to interact with multi-document summarizers is a promising direction towards improving and customizing summary results. Different ideas for interactive summarization have been proposed in previous work but these solutions are highly divergent and incomparable. In this paper, we develop an end-to-end evaluation framework for expansion-based interactive summarization, which considers the accumulating information along an interactive session. Our framework includes a procedure of collecting real user sessions and evaluation measures relying on standards, but adapted to reflect interaction. All of our solutions are intended to be released publicly as a benchmark, allowing comparison of future developments in interactive summarization. We demonstrate the use of our framework by evaluating and comparing baseline implementations that we developed for this purpose, which will serve as part of our benchmark. Our extensive experimentation and analysis of these systems motivate our design choices and support the viability of our framework.

==> figures/graphCurve.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\columnwidth]{figures/AUC_graph.pdf}
    \caption{The recall-curves and AUC scores of the average upper and lower bound sessions, and those of real sessions. The two systems' real sessions' average indeed fall between the upper and lower bound, but do not indicate any overall difference between themselves. AUC intervals are computed at $95\%$ confidence (bootstrapped \citep{Wessa2020BootstrapTool}).}
    \label{fig_curve}
\end{figure}
